TriHuman : A Real-time and Controllable Tri-plane Representation for Detailed Human Geometry and Appearance Synthesis

Creating controllable, photorealistic, and geometrically detailed digital doubles of real humans solely from video data is a key challenge in Computer Graphics and Vision, especially when real-time performance is required. Recent methods attach a neural radiance field (NeRF) to an articulated structure, e.g., a body model or a skeleton, to map points into a pose canonical space while conditioning the NeRF on the skeletal pose. These approaches typically parameterize the neural field with a multi-layer perceptron (MLP) leading to a slow runtime. To address this drawback, we propose TriHuman a novel human-tailored, deformable, and efficient tri-plane representation, which achieves real-time performance, state-of-the-art pose-controllable geometry synthesis as well as photorealistic rendering quality. At the core, we non-rigidly warp global ray samples into our undeformed tri-plane texture space, which effectively addresses the problem of global points being mapped to the same tri-plane locations. We then show how such a tri-plane feature representation can be conditioned on the skeletal motion to account for dynamic appearance and geometry changes. Our results demonstrate a clear step towards higher quality in terms of geometry and appearance modeling of humans as well as runtime performance.

==> figures/suppl_albation_qual.tex <==
\begin{figure*}[!t]
\centering
\includegraphics[width=0.99\linewidth]{images/5_ablation_qual_new.jpg}
\caption{
%
\textbf{Ablation study.}
%
We qualitatively evaluate our individual design choices for novel poses in terms of image and geometry synthesis.
%
Our results demonstrate that our proposed method consistently outperforms the baselines, which shows the superiority of our method.
%
}
\label{fig:supplqualablation}
\end{figure*}

==> sections_sup/6_applications.tex <==
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\section{Application} \label{supplsec:application}
%
In this section, we will explore additional applications enabled by Trihuman.
%
As highlighted in the main paper, Trihuman's ability to generate detailed geometry with consistent triangulation opens up new possibilities for a broad spectrum of downstream applications. 
%
Here, we will use consistent texture editing as an illustrative example of applications enabled by Trihuman.
%
\input{figures/suppl_application}
%
Figure ~\ref{fig:supplapplication} presents the results for consistent texture editing backed by Trihuman, which can be achieved from the following step:
%
Firstly, we may draw an icon with an alpha channel, serving as the texture map for the character's template mesh.
%
Next, we can render both the texture color and the alpha value through the rasterization process applied to the textured template mesh.
%
Finally, we may get consistent texture editing results by alpha-blending the neural-rendered character imagery with the rasterized icon.
%
Notably, thanks to the high-fidelity and consistent geometry generated by Trihuman, in the result after the edits, the rendered icon follows the wrinkle deformation of the clothing. 
%
Moreover, the edited result effectively retains the occlusions resulting from different poses.
